Detection of Adversarial Training Examples in Poisoning Attacks through Anomaly Detection

Machine learning has become an important component for many systems and applications including computer vision, spam filtering, malware and network intrusion detection, among others. Despite the capabilities of machine learning algorithms to extract valuable information from data and produce accurate predictions, it has been shown that these algorithms are vulnerable to attacks. Data poisoning is one of the most relevant security threats against machine learning systems, where attackers can subvert the learning process by injecting malicious samples in the training data. Recent work in adversarial machine learning has shown that the so-called optimal attack strategies can successfully poison linear classifiers, degrading the performance of the system dramatically after compromising a small fraction of the training dataset. In this paper we propose a defence mechanism to mitigate the effect of these optimal poisoning attacks based on outlier detection. We show empirically that the adversarial examples generated by these attack strategies are quite different from genuine points, as no detectability constrains are considered to craft the attack. Hence, they can be detected with an appropriate pre-filtering of the training dataset.

==> Sections/Section3_old.tex <==
\section{Background}
In a poisoning attack, the adversary injects examples in the learner's training set to influence the selection of the classifier according to a specific goal. Typically, the attacker injects examples driving the learning algorithm towards a classifier with a large classification error. Poisoning is then performed by solving an optimization problem where the poisoning examples are the decision variables and the attacker's goal is the objective. The poisoning points must lie within a feasible domain determined both by the \emph{instance space} and optionally by the constrains dictated by the attacker's necessity to stay undetected. For example, if the attacker is aware of an underlying outlier detection, poisoning should account for it and produce examples that are undetected. 

\textbf{Problem Formulation.} Formally, let $\X$ be the instance space, $\Y = \{-1, +1\}$ be the label space and $\Z = \X \times \Y$ be the example space. Given a training set\footnote{$S$ is typically called training set, however it is a training sequence as it can contain also duplicated examples. In the following we will engage a slight abuse of notation indicating sequences with the set notation.} $S$ of size $n$, a learner outputs a classifier $h_S : \X \rightarrow \Y$ from a set $\mathcal{H}$ called \emph{hypothesis class}. We consider learners which are based on the minimization of some objective function $O_L: \Z \times \H \times \R_+^k \rightarrow \R$. This class of learners includes the \emph{Empirical Risk Minimization} (ERM) and \emph{Regularized Loss Minimization}\footnote{In ERM the objective does not have a regularization term, in out formulation this can be formalized by setting the regularization parameter to 0.} paradigms. The attacker aims to inject $q$ examples $P = \{\textbf{z}_1,...,\textbf{z}_q\}$ in the defender's training set such that the objective $O_A: \Z \times \H \rightarrow \R$ is maximized. If $\hat{S} = S \cup P$ denotes the corrupted dataset, then the a poisoning attack is formalized by the following bi-level optimization problem:

\begin{equation}
\begin{aligned}
\underset{P \in \mathcal{F}^q, h_{\hat{S}}}{\max}\quad & O_A(P, h_{\hat{S}}) \\
\text{s.t.}\quad & h_{\hat{S}} \in \underset{h \in \H}{\argmin} & & O_L(\hat{S}, h, \bm{\lambda}) \\
\end{aligned}
\label{eq3:1}
\end{equation}
%
where $\mathcal{F} \triangleq \{\bm{z} \in \Z: d_i(\bm{z}) \le \bm{0} \wedge d_e(\bm{z}) = \bm{0}\}$ and $d_i:\Z \rightarrow \mathbb{R}^{i}$ and $d_e:\Z \rightarrow \mathbb{R}^{e}$ model the detectability constraints. Poisoning takes place as the classifier $h_{\hat{S}}$ is learned on the corrupted dataset.

This formulation is very general and allows to define many attack scenarios. For example, to perform an unconstrained attack where the attacker is only limited by the instance space $\mathcal{X}$ one needs to remove the detectability constraints. By contrast, an outlier detector can be modeled by some inequality constraint. For example, the presence of a distance-based outlier detector can be modeled using some inequality on euclidean distances. A simpler constrained attack, is label flipping, where the attacker is only allowed to modify the labels leads to define the feasible domain as $S \times \Y$. Finally, note that this formulation is slightly different from the one proposed by \cite{mei2015using}. Indeed, the problem in \Cref{eq3:1} does not require the attacker to have in mind a specific hypothesis as in the machine teaching context. The knowledge of such an hypothesis is unrealistic in some cases. For example, if the attacker goal is to produce a classifier with the largest classification error given the constraints, unless the underlying data distribution is know, estimating such hypothesis requires the solution of another learning task.

\textbf{Solving the Bi-level Problem.} The problem in \ref{eq3:1} is a bi-level optimization problem where the objective is named \emph{outer problem} and the constraint is named \emph{inner problem}. Bi-level optimization is NP hard in general \cite{bard2013practical}, however in many cases of interest can be with a gradient ascent strategy. Here we describe the approach proposed by \cite{mei2015using}. The approach is suitable when $O_L$ is convex and regular, in these cases the inner problem is replaced by its \emph{Kuhn-Karush-Tucker} (KKT) conditions. \Cref{eq3:1} then becomes

\begin{equation}
\begin{aligned}
\underset{P \in \mathcal{F}^q, h_{\hat{S}}}{\max}\quad & O_A(P, h_{\hat{S}}) \\
\text{s.t.}\quad & \frac{\partial O_L}{\partial h}(\hat{S}, h, \bm{\lambda}) = \bm{0} \\
\end{aligned}
\label{eq3:2}
\end{equation}
%
This problem can now be tackled with a gradient ascent strategy to find a local maximizer. The update rule at $t$-th step is given by

\begin{equation}
P^{(t+1)} = \Pi_{\F^q}(P^{(t)} + \eta^{(t)}\frac{\partial O_A}{\partial P}(P^{(t)}, h^{(t)}))
\label{eq3:3}
\end{equation}
%
where $\Pi_{A}: \Z^q \rightarrow A$ is the projection operator that ensure the feasibility of each iteration, and $\eta^{(t)}$ is a suitably chosen step-size. They key quantity to calculate in \Cref{eq3:3} is the gradient of the attacker's objective, which is given by

\begin{equation}
\frac{\partial O_A}{\partial P}(P_0, h_0) = \frac{\partial h}{\partial P} (P_0) \frac{\partial O_A}{\partial h} (P_0, h_0)
\label{eq3:4}
\end{equation}
%
The difference with respect to a standard gradient ascent approach is the presence of the Jacobian $\frac{\partial h}{\partial P}$. Indeed, for many machine learning algorithm there is not an explicit relation between the selected hypothesis and the training set. However, note that the KKT conditions for the inner problem define an implicit function $f$ between the learned hypothesis and the variables $P$, i.e. $f(P, h) = \bm{0}$. When $f$ is differentiable w.r.t. $P$ and $h$ and the Jacobian $\partial f/\partial h$ is a full-rank matrix, then the \emph{implicit function theorem} guarantees the existence of a function $i$ such that $h = g(P)$ and

\begin{equation}
\frac{\partial h}{\partial P} (P_0) = - \left[\frac{\partial f}{\partial h}(P_0, h_0) \right]^{-1} \frac{\partial f}{\partial P}(P_0, h_0)
\label{eq3:5}
\end{equation} 
%
which provides the required Jacobian. Note that although the above equation provide the exact Jacobian of $h$ w.r.t. $P$, in practice computing the inverse can be both very expensive and affected by numerical instability issues. Alternative approaches to compute or approximate this Jacobian are an research problem; we will elaborate further on this in the conclusions.

